Visualizing Causality in Mixed Reality for Manual Task Learning: An Exploratory Study

Mixed Reality (MR) is gaining prominence in manual task skill learning due to its in-situ, embodied, and immersive experience. To teach manual tasks, current methodologies break the task into hierarchies (tasks into subtasks) and visualize the current subtask and future in terms of causality. Existing psychology literature also shows that humans learn tasks by breaking them into hierarchies. In order to understand the design space of information visualized to the learner for better task understanding, we conducted a user study with 48 users. The study was conducted using a complex assembly task, which involves learning of both actions and tool usage. We aim to explore the effect of visualization of causality in the hierarchy for manual task learning in MR by four options: no causality, event level causality, interaction level causality, and gesture level causality. The results show that the user understands and performs best when all the level of causality is shown to the user. Based on the results, we further provide design recommendations and in-depth discussions for future manual task learning systems.

==> texes/scrap.tex <==
% \begin{table}[]
% \caption{TODO: Caption of this table}
% \label{tab:task}
% \begin{tabular}{|p{0.08\linewidth}|p{0.02\linewidth}|p{0.15\linewidth}|p{0.15\linewidth}|}
% \hline
% Event                                           &  No.  & Interactions                                     & Objects involve in interaction       \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Fix base\\ on desk\end{tabular}}                 & 1  & Move a base panel up onto a table                & Base, desk                           \\ \cline{2-4} 
%                                                   & 2  & fix the base panel with clamp A                  & Base, desk and clamp A               \\ \cline{2-4} 
%                                                   & 3  & fix the base panel with clamp B                  & Base, desk and clamp B               \\ \cline{2-4} 
%                                                   & 4  & Strike hammer to check the stability of base     & Hammer, base and clamp A and Clamp B \\ \hline
% \multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Print\\ Ruler\\ from a 3D\\ printer\end{tabular}} & 5  & Rotate the printer                               & Printer                             \\ \cline{2-4} 
%                                                   & 6  & Attach PVA to printer                            & PVA and Printer                      \\ \cline{2-4} 
%                                                   & 7  & Attach PLA to printer                            & PLA and Printer                      \\ \cline{2-4} 
%                                                   & 8  & Attach HIPS to printer                           & HIPS and Printer                     \\ \cline{2-4} 
%                                                   & 9  & Insert hard drive to load CAD model              & Hard drive and printer               \\ \cline{2-4} 
%                                                   & 10 & Press Start button                               & Printer                              \\ \cline{2-4} 
%                                                   & 11 & Pick ruler from printer                          & Ruler and printer                    \\ \hline
% \multirow{1}{*}{\begin{tabular}[c]{@{}c@{}}Install \\ Stand\end{tabular}}                                & 12 & Mark 12 inch from the end on the base with ruler & Ruler, base and base                 \\ \hline
% \end{tabular}
% \hfill
% \begin{tabular}{|p{0.08\linewidth}|p{0.02\linewidth}|p{0.15\linewidth}|p{0.15\linewidth}|}
% \hline
% Event                             &  No.  & Interactions                                  & Objects involve in interaction \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Install \\ Stand\end{tabular}} & 13 & Move the bolt to the location                 & Screwdriver and bolt           \\ \cline{2-4} 
%                                     & 14 & Align the stand to the bolt                   & Stand and bolt                 \\ \cline{2-4} 
%                                     & 15 & Fix the stand with screwdriver                & Screwdriver,stand and base     \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Install \\ Arm\end{tabular}}   & 16 & Mark 12 inch on stand from the top with ruler & Ruler, stand and base          \\ \cline{2-4} 
%                                     & 17 & Slide the arm to the location                 & Arm and stand                  \\ \cline{2-4} 
%                                     & 18 & Fix the arm to the stand                      & Screwdriver, stand and arm     \\ \hline
% \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Install \\ Mount\end{tabular}} & 19 & Slide the mount into the arm                  & Mount and arm                  \\ \cline{2-4} 
%                                     & 20 & Fix the mount with screwdriver                & Screwdriver mount and stand    \\ \cline{2-4} 
%                                     & 21 & Align board with mount                        & Board and mount                \\ \cline{2-4} 
%                                     & 22 & Drill two holes on the board                  & Drill gun and board            \\ \cline{2-4} 
%                                     & 23 & Screw the bolts                               & Wrench, bolts and boards       \\ \hline
% \multirow{1}{*}{\begin{tabular}[c]{@{}c@{}}Attach \\ Camera\end{tabular}}                    & 24 & Attach Camera to Mount                        & Camera, Mount                  \\ \hline
% \end{tabular}
% \end{table}
